TAIA: Large Language Models are Out-of-Distribution Data Learners

Fine-tuning on task-specific question-answer pairs is a predominant method for enhancing the performance of instruction-tuned large language models (LLMs) on downstream tasks. However, in certain specialized domains, such as healthcare or harmless content generation, it is nearly impossible to obtain a large volume of high-quality data that matches the downstream distribution. To improve the performance of LLMs in data-scarce domains with domain-mismatched data, we re-evaluated the Transformer architecture and discovered that not all parameter updates during fine-tuning contribute positively to downstream performance. Our analysis reveals that within the self-attention and feed-forward networks, only the fine-tuned attention parameters are particularly beneficial when the training set's distribution does not fully align with the test set. Based on this insight, we propose an effective inference-time intervention method: Training All parameters but Inferring with only Attention (\trainallInfAttn). We empirically validate \trainallInfAttn using two general instruction-tuning datasets and evaluate it on seven downstream tasks involving math, reasoning, and knowledge understanding across LLMs of different parameter sizes and fine-tuning techniques. Our comprehensive experiments demonstrate that \trainallInfAttn achieves superior improvements compared to both the fully fine-tuned model and the base model in most scenarios, with significant performance gains. The high tolerance of \trainallInfAttn to data mismatches makes it resistant to jailbreaking tuning and enhances specialized tasks using general data. Code is available in \url{https://github.com/pixas/TAIA_LLM}.

==> deprecated.tex <==
we put forward two attempts to mitigate the noisy knowledge injected into FFN:
\begin{enumerate}[itemsep=0.8mm, parsep=0pt, leftmargin=*]
    \item [\ding{192}] We directly fine-tune the LLM on its self-attention part and freeze other parts. This practice maintains the parameterized knowledge uninfluenced. We call it as~\trainAttn~(\uline{T}rain \uline{Attn}).
    \item [\ding{193}] We follow vanilla fine-tuning to add all parameters into the optimizer group. Instead, we only maintain the updated self-attention part and reuse the pretrained weights for FFN modules, which we name as~\trainallInfAttn~(\uline{T}rain-\uline{A}ll-\uline{I}nfer-\uline{Attn}).
\end{enumerate}
We separately compare these two attempts with the baseline:

\paragraph{\trainAttn versus the baseline}
Fine-tuning only partial parameters has already become a widely used methodology to achieve a trade-off between performance and training efficiency thanks to the superfluity of parameters~\citep{hu2021lora,yu2023language}.
\syj{in this paragraph, we state that although train-attn is as good as train all, but train only attn will make the optimization space smaller, which can prompt the optimization process unstable and suboptimal when given OOD data}

\paragraph{\trainallInfAttn versus the baseline}
\syj{use the original statement (sft learns the instruction-following ability and the ffn parameters bring unnecessary knowledge perturbation for base models, which can provide bad effects.)}

\paragraph{\trainallInfAttn versus \trainAttn}
\syj{cite attention is not all you need and show formulation of the rank collapse. show the rank-layer diagram here.}

Thus, after standard fine-tuning, it proves more advantageous to maintain the updated parameters related to self-attention while discarding those learned by the FFN to mitigate catastrophic forgetting. 
This novel approach significantly enhances the adaptability of LLMs across various domains when dealing with OOD fine-tuning data.
We rename this strategy as \uline{T}rain-\uline{A}ll-\uline{I}nfer-\uline{ATT}entio\uline{N}~(TA-I-ATTN).

% \paragraph{Orthogonal Capabilities of Self-Attention and FFN}
% We here systematically evaluate the orthogonal efficacy of the self-attention and feed-forward networks using four settings: train-only-attention~(T-attn), train-only-ffn~(T-ffn), train-all-infer-only-attention~(TA-I-attn), and train-all-infer-only-ffn~(TA-I-ffn), as well as the baseline, train-all-infer-all.
% We choose \texttt{Qwen1.5-1.8b-chat}~\citep{qwen} as the seed LLM for fine-tuning.
% \syj{leave for sheng}

\paragraph{Broader Data Generalization: An Activation Similarity View}
The above analysis shows that when trained on task-specific training data, the TA-I-ATTN utilizes the principle goal of supervised fine-tuning towards a superior downstream adaptation.
Based on this strategy, the fine-tuned models can exhibit significant generalization ability when fine-tuned on held-out tasks, since the pretrained knowledge stored in FFNs has never been distracted.
% To theoretically validate the efficacy of TA-I-ATTN, we 
We here examine the generalization of the TA-I-ATTN setting from a perspective of activation similarities.
We define the activation similarity of the $i$-th data sample between two models $\boldsymbol{\theta}_p$ and $\boldsymbol{\theta}_q$ trained separately on two corpus $D_p \sim P, D_q \sim Q$ as such:
\begin{equation}
    \mathrm{Sim}(\mathbf{h}_p,\mathbf{h}_q)_i=\frac{1}{L}\sum_{l=1}^L \frac{\mathbf{h}_{pi}^{l\top} \mathbf{h}_{qi}^l}{\|\mathbf{h}_{pi}^l\|\cdot \|\mathbf{h}_{qi}^l\|}
\end{equation}
where $\mathbf{h}_p,\mathbf{h}_q$ are the activation hidden states after certain modules, and $L$ is the number of hidden layers.
We select C-eval~\citep{huang2024c} as the test and Medical-Collection, CoT-Collection~\citep{kim-etal-2023-cot}, and a 180K subset of OpenMath~\citep{toshniwal2024openmath} as our training corpus.
We use greedy decoding and limit the output space to a single answer with logit bias~\footnote{\url{https://platform.openai.com/docs/api-reference/chat/create\#chat-create-logit_bias}} and obtain the similarity-performance correlation in Fig.~\ref{fig: overview analysis}.
It shows that the TA-I-ATTN setting leads to a higher activation similarity in most cases compared to the Train-All-Infer-FFN~(TA-I-FFN) and baseline settings.
The highest similarity of the TA-I-ATTN setting correlates to its best performance on C-eval, no matter which training corpus it uses.
It consolidates that \emph{if we prompt LLMs to emphasize the instruction-following ability instead of new knowledge through TA-I-ATTN, the fine-tuned models demonstrate robust generalization performance and transferability of training data. }
